Poisoning Attacks on Algorithmic Fairness

Research in adversarial machine learning has shown how the performance of machine learning models can be seriously compromised by injecting even a small fraction of poisoning points into the training data. While the effects on model accuracy of such poisoning attacks have been widely studied, their potential effects on other model performance metrics remain to be evaluated. In this work, we introduce an optimization framework for poisoning attacks against algorithmic fairness, and develop a gradient-based poisoning attack aimed at introducing classification disparities among different groups in the data. We empirically show that our attack is effective not only in the white-box setting, in which the attacker has full access to the target model, but also in a more challenging black-box scenario in which the attacks are optimized against a substitute model and then transferred to the target model. We believe that our findings pave the way towards the definition of an entirely novel set of adversarial attacks targeting algorithmic fairness in different scenarios, and that investigating such vulnerabilities will help design more robust algorithms and countermeasures in the future.

==> attack_impact_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\begin{tabular}{cl|l|l|l|l|l|l|l|}
\cline{3-9}
\multicolumn{1}{l}{}                                                                                         &                                                                                    & \textbf{Accuracy} & \textbf{\begin{tabular}[c]{@{}l@{}}Demographic \\ parity\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Avg. odds \\ difference\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}FNR \\ privileged\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}FNR \\ unprivileged\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}FPR \\ privileged\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}FPR \\ unprivileged\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Synthetic \\ dataset\end{tabular}}}} & \begin{tabular}[c]{@{}l@{}}Perfect Knowledge\\  (white-box)\\  attack\end{tabular} & 0.968             & 1.962                                                                  & 2.780                                                                    & 0.367                                                              & 0.873                                                                & 3.176                                                              & 2.034                                                                \\ \cline{2-9} 
\multicolumn{1}{|c|}{}                                                                                       & \begin{tabular}[c]{@{}l@{}}Zero Knowledge \\ (black-box) attack\end{tabular}       & 0.989             & 1.683                                                                  & 2.327                                                                    & 0.308                                                              & 0.666                                                                & 2.426                                                              & 1.846                                                                \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Compas \\ dataset\end{tabular}}}}    & Perfect Knowledge (white-box) attack                                               & 0.814             & 2.355                                                                  & 3.102                                                                    & 0                                                                  & 2.274                                                                & 1.846                                                              & 0.477                                                                \\ \cline{2-9} 
\multicolumn{1}{|c|}{}                                                                                       & Zero Knowledge (black-box) attack                                                  & 0.899             & 1.731                                                                  & 2.297                                                                    & 0                                                                  & 1.456                                                                & 1.824                                                              & 0.906                                                                \\ \hline
\end{tabular}
\caption{}
\label{tab:performance_comparison}
\end{table}

==> old_sections/00-abstract.tex <==
\begin{abstract}
Research in adversarial machine learning has shown how the performance of machine learning models can be seriously compromised by small perturbations in the training data.
While the effects on model accuracy of adversarial attacks have been widely studied in the field, their potential effects on other model performance metrics remains to be evaluated.
In this work, we introduce a theoretical analysis of how state of the art on adversarial machine learning attacks can be adapted to compromise a supervised classifiers from the perspective of algorithmic discrimination.
We then empirically test the effects of adversarial attacks, crafted with the purpose of increasing disparate impact and disparate mistreatment, two common measures used to evaluate algorithmic discrimination. %, across different groups.
Our results show how classification disparities can be introduced or exaggerated through small changes in the input data and under limited previous knowledge from the attacker.
%
\keywords{algorithmic discrimination \and algorithmic fairness \and poisoning attacks \and adversarial machine learning \and  machine learning security}
\end{abstract}

==> old_sections/01-introduction.tex <==
%!TEX root = paper.tex

\begin{abstract}
Research in adversarial machine learning has shown how the performance of machine learning models can be seriously compromised by small perturbations in the training data.
%
While the effects on model accuracy of adversarial attacks have been widely studied in the field, their potential effects on other model performance metrics remains to be evaluated.
%
In this work, we introduce a theoretical analysis of how different types of adversarial machine learning attacks can be crafted to compromise a supervised classifiers from the perspective of algorithmic discrimination.
%
We then empirically test the effects of two different adversarial attacks, crafted with the purpose of increasing disparate impact and disparate mistreatment, two common measures used to evaluate algorithmic discrimination. %, across different groups.
%
Our results show how classification disparities can be introduced or exaggerated through small changes in the input data and under limited previous knowledge from the attacker.
%
\keywords{algorithmic discrimination \and algorithmic fairness \and adversarial machine learning attacks}
\end{abstract}

\section{Introduction}
The literature on Adversarial Machine Learning has described several types of adversarial attacks crafted with the purpose of increasing the misclassification rate in a machine learning model, either for certain samples or in an indiscriminate basis (see, e.g., \cite{biggio2018wild}).
%
In this work, we explore how analogous techniques can be used to compromise a machine learning model, not to drive its accuracy down, but with the purpose of adding algorithmic discrimination, or exaggerating it if it already exists. In other words, the purpose of the attacker will be to create or increase a disadvantage against a specific group of individuals or samples.

\subsection{Motivation}

The main goal of this paper is to show the potential harm that an attacker can cause in a machine learning system if the attacker can manipulate its training data.
%
For instance, the developer of a criminal recidivism prediction tool~\cite{ProPublica_article} could sample training data in a discriminatory manner to bias the tool against a certain group of people.
%
Similar harms can occur when training data is collected from public sources, such as surveys done online that cannot be fully trusted.
%
A minority of ill-intentioned users could \emph{poison} this data with the objective of causing certain defects in the machine learning system created from it.


In addition to these examples, there is the unintentional setting, % which arguably could be considered more realistic,
% -- I think the intentional setting is also realistic --ChaTo
where inequities are introduced in the machine learning model as an undesired effect of the data collection or data labeling.
%
For instance, human annotators could systematically make mistakes when assigning labels to images of people of a certain skin color~\cite{buolamwini2018}.


The methods we describe on this paper could be used to model the potential harm to a machine learning system in the worst case scenario, demonstrating the undesired effects that a limited amount of wrongly labeled samples can cause, even if created in an unwanted manner.

\subsection{Contributions}

This work first characterizes several types of possible adversarial attacks that could be crafted with the purpose of introducing algorithmic discrimination in a model.
%
Different types of attacks are defined in terms of the attacker knowledge,  capabilities, and strategy.


After this characterization, we perform experiments in two scenarios: a ``black-box'' attack in which the attacker only has access to the training data, but not the model, and a ``white-box'' scenario in which the attacker has access to the model.
%
The effects of these attacks are measured using impact quantification metrics.
%
The experiments show that by carefully perturbing a limited amount of training examples, an skilled attacker has the possibility of introducing different types of inequities for certain groups of individuals.
%
This, can be done without large effects on the overall accuracy of the system, which makes these attacks harder to detect.


The rest of this paper is organized as follows.
%
Section~\ref{sec:background}, provides background on adversarial machine learning and algorithmic fairness.
%
Section~\label{sec:attack-models} describes how an existing categorization of different types of adversarial machine learning attacks can be extended to fit with the new type of attacks introduced in this paper.
%
Section~\label{sec:experiments} demonstrates empirically the feasibility of the new types of attacks on both synthetic and real-world data.
%
Section~\label{sec:related-work} provides further references to related work.
%
Section~\label{sec:conclusions} presents our conclusions and future work.


==> old_sections/02-background.tex <==
%!TEX root = paper.tex

\section{Background}\label{sec:background}

In this section we provide an overview those research contributions research done in the fields of \textit{Adversarial Machine Learning} and \textit{Algorithmic Fairness} that are more closely related to the contribution of this paper.
\newline
\newline
\subsection{Adversarial machine learning}
The topic of Adversarial Machine Learning studies how adversarial samples can be crafted to fool machine learning models. Starting from 2004 \cite{adversarial_classification_2004}, when it was introduced in the context of spam filtering models and evolving with the new techniques, different works have proved how even high performance models from different domains such as natural language processing \cite{aversarial_learning_2005}, object recognition in images \cite{goodfellow2014explaining,nguyen2014deep,moosavidezfooli2015deepfool} or malware detection \cite{aversarial_learning_2005} can be easily fooled by adversarial examples. Adversarial examples are carefully-perturbed input samples aimed to mislead detection at test time \cite{Biggio_2018}.

Although explainability techniques are being adopted to understand and validate how autonomous models are taking their decisions, recent work \cite{slack2019fool} has also shown that such techniques are also vulnerable against poisoning attacks. Adversarial attacks have also been used in algorithmic fairness \cite{slack2019fool,Kulynych_2020} as pre-processing techniques for mitigating unfairness and biases.

In general, literature in adversarial attacks differentiates between (a) poisoning attacks and (b) evasion attacks. Where the first are crafted by modifying input data to perturb the learned function, the later are focused on modifying samples to evade detection at test time.

This work focuses on poisoning attacks. As explained in \cite{Biggio_2018}, Poisoning attacks are generally formulated as bilevel optimization problem in which the outer optimization maximizes the attacker's objective $\set A$ for the validation set of data $D_{val}$. while the inner optimization maximizes the model learning from the input data by minimizing the error as measured by a loss function $\set L$ on the training dataset $D_{tr}$. Following this explanation, the problem is formulated as:

\begin{align}
  \label{eqObjective1} \set D_c^{\star} \in & \argmax_{\set D_{c}^{\prime} \in \Phi(\set D_{c})} && \set A(\set D_{c}^{\prime}, \vct \theta) = L ({\set D}_{\rm val}, {\vct w^\star}) \, ,  \\
 \label{eqObjective2} &{\rm s.t.}   && {\vct w^\star} \in \argmin_{\vct w^{\prime} \in \set W} \set L({\set D}_{\rm tr} \cup \set D_{c}^{\prime}, \vct w^{\prime}) \, ,
\end{align}.
\newline
\newline
\subsection{Algorithmic fairness}
During the past few years, the intersection between data mining, machine learning and fairness domains has received an increasing attention by the research community. In this context, the work done for task of quantifying inequities, named algorithmic fairness, resulted in a multitude of metrics to quantify fairness.\\

The existing metrics of fairness for classification fall in two categories:  \textit{Individual metrics} and \textit{Group metrics} depending if the goal is to require the system to give similar predictions to individuals that are considered similar or the objective is that the system treats groups equally. The groups are often calculated in the bases of sensible attributes that are legally recognized as protected classes.\\

In general, approaches to algorithmic fairness are based on a specific distribution of the feature space. As indicated by \cite{Pedreschi_2012}, this distribution can be expressed in the form of a contingency table that divides the features space in terms of the groups found in the data. Groups are calculated with respect to a protected attribute $A$ and a target variable $Y$, for which some of the possible values are considered more beneficial than others. Following this ideas, for the simple case of binary classification and two groups, the feature space is divided as depicted in Table \ref{tab:fairness_feature_space}.


\begin{table}[ht!]
\centering
\begin{tabular}{llllll}
                                                           &                                  & \multicolumn{2}{c}{{\ul \textbf{benefit}}}                 &    &  \\ \cline{3-4}
                                                           & \multicolumn{1}{l|}{}            & \multicolumn{1}{l|}{denied} & \multicolumn{1}{l|}{granted} &    &  \\ \cline{2-5}
\multicolumn{1}{c|}{\multirow{2}{*}{{\ul \textbf{group}}}} & \multicolumn{1}{l|}{unprivileged}   & \multicolumn{1}{l|}{$u^-$}      & \multicolumn{1}{l|}{$u^+$}       & $n_1$ &  \\ \cline{2-5}
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{l|}{privileged} & \multicolumn{1}{l|}{$p^-$}      & \multicolumn{1}{l|}{$p^+$}       & $n_2$ &  \\ \cline{2-5}
                                                           & \multicolumn{1}{l|}{}            & \multicolumn{1}{l|}{$m_1$}     & \multicolumn{1}{l|}{$m_2$}      & $n$  &
\end{tabular}
\medskip
\caption{Contingency table. Distribution of feature space in algorithmic fairness literature}
\label{tab:fairness_feature_space}
\end{table}


As proposed in the literature \cite{alex2016fair,Zafar_2017,feldman2015}, fairness functions are defined by using the criteria of \textit{disparate impact} and \textit{disparate misclasification} depending on the final goal of the metric.

Given $X$, a feature vector representing individuals; $A$, a sensitive attribute; $C$, a predictor and $Y$ a target variable, the stated criteria are defined as follows:
\begin{itemize}
    \item {\textbf{Disparate impact:} Requires $C$ independent of $A$ ($C\perp A$).\\ Implies that for all groups $a$, $b$ and all values $y$, $P_a (C=y) = P_b(C=y) $.\\
    This criterion ignores possible correlations between $Y$ and $A$.\\ The case of the perfect predictor ($C = Y$) is in general not accepted in most cases, where initial rates for $Y$ values across groups are not equalized. \\
    Examples of metrics based in this criteria are: \textit{demographic parity} and \textit{statistical parity}.}\\

    \item {\textbf{Disparate mistreatment:} Requires $C$ independent of $A$ conditional on $Y$ ($C\perp A | Y$)}.\\
    This criteria incentives to reduce errors uniformly in all groups. The case of the perfect predictor $C = Y$ is allowed and corresponds to the ideal scenario. Introduced first in \cite{Zafar_2017}, examples of metrics based on it are: \textit{true positive ratio}, \textit{false positive ratio}, \textit{false negative ratio} that for the best case scenario should be equalized for the obtained groups.\\
\end{itemize}

The impossibility theorem of satisfying any both criteria at the same time is already known. In  \cite{alex2016fair,kleinberg2016}, authors demonstrated the unfeasibility of achieving fairness according both definitions at the same time, when the base rates for the different groups is different.

\begin{comment}
\subsection{Contribution of this work}
\todo{It is repetitive to explain the contribution here again. This should go in the introduction --ChaTo}
This work is framed in the intersection between Adversarial Machine Learning and Algorithmic Fairness. The main contribution is the proposal of a new type of adversarial attacks that we call \textit{Adversarial Fairness Attacks}.

The main characteristic of this novel type of attack is they are crafted with the objective of increasing the unfairness of the system. Next section describes the characteristics of the different models of Adversarial Fairness Attacks.
\end{comment}

==> old_sections/03-attack-models.tex <==
%!TEX root = paper.tex

\section{Adversarial Fairness Attack Models}

This section describes a taxonomy of different varieties of adversarial attacks that could be crafted to compromise algorithmic fairness. The characterization is based and extended from the taxonomy proposed in \cite{Biggio_2018} where attacks are defined by the goal of the attacker, the knowledge the attacker has about the system, the capabilities of the attacker, her strategy and the approach used to measure the impact of a given attack.

In this taxonomy, only \textit{poisoning attacks} are considered, as it's not clear how \textit{evasion attacks} could be linked to the fairness literature.
%% Attacker's goal
\subsection{Attacker’s Goal}
The goal of the attacker is represented in terms of the desired security violation, specificity of the attack and the specificity of the error.

\textbf{Security violation}: The goal of the attack can be defined as \textit{integrity violation} when the goal of the attacker is to increase disparate impact without compromising normal system operation. An specially interesting case of integrity violation attack would be the case where the goal is to increase discrimination to a level that can be punished by law, as could happen if exceeding the 80\% rule of maximum acceptable disparate impact proposed by the US Equal Employment Opportunity Commission (EEOC) \cite{feldman2015,zafar2015fairness}. An \textit{availability violation} goal would apply in setups where the objective is to compromise the normal system operations available to legitimate users, by direct effect of the introduced discrimination or as indirect result of such effect.

\textbf{Attack Specificity}: The attack would be always considered a \textit{targeted} attack in the terms of adversarial ML definition of the concept, as the objective is to increase disparate impact for certain groups of samples. In addition, considering the targeted samples the attack can be \textit{group imprecise} if all the protected groups are targeted by the attack or \textit{group specific} if only a subset of the unfavorable groups are affected by the attack.

\textbf{Error Specificity}: The error introduced by this particular type of attacks is considered \textit{specific}, as the objective is always to increase the probability of assigning unfavorable outcomes or augmenting the misclassification ratio for certain groups of samples as calculated based on protected attributes.

%% Attacker's knowledge
\subsection{Attacker’s Knowledge}\label{section-3}
Literature of adversarial machine learning defines the system as a composition of the training data $\set D$, the feature set $\set X$, the learning algorithm $\set F$, the objective function $\set L$ minimized during training and for certain models, the parameters and hyper-parameters $\theta ^\star$. Assuming different sets of known parameters for the attacker,

The attacker can also have different degrees of knowledge about the context of the data and therefore, about the privileged condition of the different groups in the training, validation and/or test sets. Although this might sound complicated, state of the art on algorithmic fairness literature commonly defines sub-groups on the grounds of the Human right law's protected attributes such as race, skin color, religion, nationality, sex, gender, marital status, age and pregnancy. In the presence of such attributes, the privileged and unprivileged groups can be easily understood based on well-known historical biases reflected in the society that are more than often represented in the data.

In the other hand, in the presence of a multitude of definitions of algorithmic fairness, the attacker might be aware of the specific metric utilized to assess the fairness of the system or the absence of such assessment which would correspond to the most usual case. Previous work has also proved that algorithmic fairness metrics are correlated in two to three families. Knowing which is the family of the fairness metric used to evaluate the system can then be enough to compromise the system performance from the perspective of algorithmic fairness, as previous work proved that fairness metrics tend to be correlated \cite{friedler2018comparative}.

Depending on the knowledge of the attacker of the different parts of the system, the following scenarios are depicted:

\textbf{Perfect-Knowledge (PK) White-Box Attacks}. The attacker is assumed to know everything about the system. This setting would correspond to the worst-case scenario, where maximum-impact biases could be adversarially added at multiple levels of the system to maximize disparate impacts.


\textbf{Limited-Knowledge (LK) Gray-Box Attacks}.
Different settings can be considered depending on the attacker's knowledge about each component of the system. Between the components the attacker might be assumed to know, there are the feature representation $\set X$ and the kind of learning algorithm $\set F$. The attacker might also be aware of the model parameters $\theta^\star$, or the training data set $\set D_{tr}$ used to create the model. In the case of the attacker not having access to the training data set $\set D_{tr}$, the attacker might be able to collect a surrogate data set $\set {D}_{tr}'$ from a similar source.

At the same time, the attacker can have different degrees of knowledge about the protected attributes present in the data or in the underlying population from which the data was gathered.

\textbf{Zero-Knowledge (ZK) Black-Box Attacks}. Some work in the context of Adversarial Machine Learning proving that a machine learning system can be compromised without any a-priori knowledge of the feature space, learning algorithm and training data has been recently published. This type of attacks assume in any case that the attacker knows the task that the system is solving and as explained in the case above, one might assume that possible biases coming from historical discrimination can be easily suspected by the attacker and therefore, knowledge from historical biases and societal prejudices can be used to craft an idea of which unpriviledged groups can be found in the population the system has access to. Using such information, an idea of potential transformations that could be used to maximize differences can be formed.


%%In the experiments section, we compare the case of the attacker having access to the training data with the case of the attacker only having knowledge of the training data.

%% Attacker's capability
\subsection{Attacker’s Capability}.
The attacker's capability defines the influence that the attacker has on the input data and, if applicable, the scenario-specific data manipulation constrains.

\textbf{Attack influence}. According to previous literature, the attacker can influence both training and test data or only test data, respectively exercising a \textit{causative} or \textit{exploratory} influence. This types of attacks have also been referred as \textit{poisoning} and
 \textit{evasion} attacks respectively. As has been said previously, this work is only focused in {poisoning attacks} where the attacker aims to inject well-crafted poisoning points into the training data to maximally compromise the output of the system.

\textbf{Data manipulation constraints}. Generally speaking, data manipulation constrains are given by the domain and context of the application to evade detection. This constraints define the space of possible data modifications.

In the experiments section, a type of attack with the constrain of not generating fake data, but sampling from the original distribution is utilized.

%% Attacker's impact
\subsection{Attacker’s Strategy}
Given the attacker's knowledge and capability, the attacker's goal can be defined as objective function.


\begin{comment}
%% Attack impact
\subsection{Attack impact measurement}
The impact of the attack is quantified by measuring the performance obtained for the model trained using the original training data set ($M_1$) and for the model trained using the adversarial samples ($M_2$). The impact can be measured as the difference for such models on the following metrics:

\textbf{Balanced accuracy}.Following earlier fairness-aware approaches, in this work we measure classier performance using balanced accuracy, i.e. the average proportion of correctly classified samples calculated for each group of samples individually.

\textbf{Disparate impact}.We calculate the impact of the attack by comparing the disparate impact observed in the models $M_1, M_2$.

Both metrics are measured for different classification thresholds (also called decision thresholds). Performance for the different thresholds can be compared by:
\begin{itemize}
    \item{\textbf{Differences of areas between the curves} can be compared for the models $M_1, M_2$. Scenarios with smaller areas between the disparate impact curves of such curves are considered to be more robust against the adversarial disparate impact attacks. The area between the accuracy curves tends to be minimized by the problem definition.}
    \item{\textbf{Maximum difference} in balanced accuracy and disparate impact can be utilized. Only classification thresholds where balanced accuracy of $M_1$ is high enough are considered, to avoid noisy results. To filter the results using this criteria, classification thresholds for which $M_1$ has a maximum difference of $10-20\%$ with respect to the best balanced accuracy are considered.}
\end{itemize}

\end{comment}
\begin{comment}

In the following experiments, we focus the analysis on how poisoning attacks can be utilized to reduce system fairness, using the disparate impact notion. This is the best contribution focused on rafting an attack with the objective of compromising disparate impact definition of fairness, to the best of the authors knowledge.

As explained by \cite{feldman2015}, U.S. law encodes unintentional biases in the form of \textit{disparate impact}. which occurs when a decision taking process has widely different outcomes for different groups of individuals. As examples of this presence in law, Griggs v. Duke Power Co, the US Supreme Court ruled a business hiriring decision ilegal if it resulted in disparate impact by race, even if decision was not explicitly determined based on race. Ricci v. DeStefano examined the relationship between disparate impact and \textit{disparate treatement}, which refers to intended or direct discrimination. In the EU General Data Protection Regulation, the human rights law, defines as illegal to treat individuals differently because of their sex, cultural background, ethnicity, religious beliefs or family affiliation, amongst others. Although it doesn't explicitly mention disparate impact, it seems to be the metric of disparity more aligned with the stated definition of discrimination.

Disparate impact is measured in the algorithmic fairness domain as the ratio in the positive outcomes across groups. In the case if a binary classification problem, where one of the assigned outcome values is understood as favorable whereas the other possible result is therefore defined as the unfavorable outcome.

Therefore, disparate impact is measured as follows:

$$D_{imp} = \dfrac{P( Y = 1 | G = unprivileged )}{P( Y = 1 | G = privileged )} $$


%%Where:
%%$$ unprivileged_{rate} = \sum_{i=1}^n [x_i \in %%G_{unprivileged} \And y_i=1]$$
%%and $$privileged_{rate} = \sum_{i=1}^n [x_i \in %%G_{privileged} \And y_i=1]$$

%%$$D_{imp} = \dfrac{\dfrac{unprivileged_{rate}}{(unprivilege%%d_{rate} + privileged_{rate})}}{\dfrac{privileged_{rate}}{(%%unprivileged_{rate} + privileged_{rate})}}$$
%%
Where $Y$ refers to the target variable, $y_i=1$ encodes the favorable label and G refers to the groups of individuals.


Expressed in the notation introduced in Table \ref{tab:fairness_feature_space}, disparate impact can be formulated as:

$$ D_{imp} = \frac{\frac{b}{n1}}{\frac{d}{n2}} $$

Understanding that protected groups are calculated on the basis of sensible attributes that are fixed from the problem perspective, disparate impact will get maximally increased when the system doesn't grant the benefit to any member of the unprivileged or protected group and the benefit is granted for all the members of the privileged group at the same time.

\end{comment}

%%
%%Although legislation has resisted a \textit{rigid %%mathematical formula} to quantify disparate impact %%\cite{Watson_1988}, we use the generalization of the 80\% %%rule as maximum acceptable value for the disparate impact %%ratio as proposed by the US Equal Employment Opportunity %%Commission (EEOC) \cite{feldman2015, zafar2015fairness}. %%While disparate impact can be directly measured in data %%to %%calculate disparities present in the data or in %%predictions to assess impact introduced by the predictive %%algorithm, a dataset and/or a system will be defined as %%unfair if they satisfy $D_{imp} < 0.8$


The experiments have been crafted to empirically measure differences when comparing performance for models trained with the original data vs. performance for models trained using the adversarial/manipulated data. Performance is measured using the metrics explained above.


==> old_sections/04-experiments.tex <==
%!TEX root = paper.tex

\section{Experiments}\label{sec:experiments}

This section describes the obtained results for two different types of attacks. We have selected one example of a \textit{Perfect-Knowledge (PK) White-Box Attack} where the original model is fully known for the attacker. Then, we tested a set up of \textit{Limited-Knowledge (PK) Gray-Box Attack} where the attacker has access to the train data, so a surrogate model can be trained and the attack can be then optimized using the learning function of this model. This scenarios were selected

To formulate the experiments, we use the following notation: \\ \\
\textbf{Notation.} We denote the sample and label spaces with $X$ and $Y \in [0,1]$, respectively. Training data is denoted as $\set D_{tr}=(x_i, y_i)^{N}_{i=1}$, where $N$ is the training set size. $\set L(\set D,p)$ is used to denote the loss incurred by a classifier $\set F \; : \; X \rightarrow Y $ (parametrized by model parameters $ \theta^\star$). Typically, the $\set L$ is computed by averaging a loss function $\ell$ measured for each data points where $\ell(y,x,  \theta^\star)$ i.e., $\set L(\set D_{tr}, \theta^\star) = \frac{1}{N} \sum_{i=1}^{N} \ell(y_i, x_i,  \theta^\star)$\newline \newline


The following experiments were crafted by adding a maximum number of 5\% of poisoned samples. And results are compared between a linear model and a non-linear one, to ensure effects are not consequence of the limited complexity of the learned function.
The objective of the attacker is then to add a set of points $\mathbf{x'}$ whose addition to $\set D_{tr}$ maximally increase the disparate impact $D_{imp}$ of the system as measured in the validation data set $\set D_{val}$.

Using the notation above and adapting the classic equations used to formulate poisoning attacks Eq.\ref{eqObjective1} and Eq.\ref{eqObjective2} the optimal attack strategy can be formulated as a bilevel optimization problem as follows:
\begin{eqnarray}
    \label{eq:obj-pois}
    \max_{\vct x^\prime} & & \sum_{k=1}^p \ell (x_k, \vct y_k, \param^\star) - \lambda \sum_{j=1}^m \ell (x_j, \vct y_j, \param^\star) \\
    {\rm s.t.} & &  \param^\star \in  \argmin_{\param} \set L (\set D_{\rm tr} \cup (\vct x^\prime, y^\prime), \vct \param)
    \label{eq:poisoning_problem}
\end{eqnarray}

The validation loss (outer max problem) consists of maximizing the error on the minority group of $p$ points (indexed by $k$), while preserving the loss on the other $m$ points (indexed by $j$). The trade-off parameter $\lambda$ aims to balance the contribution of the two terms in the validation loss. \\

Also, the experiments were executed using the following characterization:\\

\subsubsection{Attack characterization}
Using the framework explained in Section \ref{section-3}, the tested attacks are characterized as follows:
\begin{itemize}
    \item{\textbf{Goal}: \textit{integrity violation} goal with the objective of increasing disparate impact or disparate mistreatment without compromising normal system operation and \textit{group imprecise}, with the purpose of increment disparate impact between all privileged groups with respect to all the unprivileged ones.}
    \item{\textbf{Knowledge}: Two different settings are considered in the experiments. In one hand, we assessed an scenario of \textit{Perfect-Knowledge (PK) White-Box attack} where he attacker is assumed to know the task the system is designed to perform, and to know an have access to the training data and its context in terms of the privileged and unprivileged groups. The learning function (algorithm) is also known so the attack can be optimized against such function. In the second experiment, we consider a setting of \textit{Limited-Knowledge (PK) Gray-Box attack} where the attacker knows the task the system is designed to perform and has access to the training data and the protected characteristics but the concrete model remains unknown for the attacker, so a surrogate model can be trained and used to approximate the original one. This is a setting where the transferability of this type of attacks \textit{demontis2018adversarial} is also stressed.
    }
    \item{\textbf{Capability}: Characterized as \textit{poisoning attack}, the attacker would add new samples to input data with the objective of altering the learning function of the system to increase the disparate impact of subsequent model predictions.}
    \item{\textbf{Strategy}: The strategy implemented to craft the attacks is constrained to a maximum number of 5\% poisoned samples added to the training data.}

\end{itemize}

\subsection{Disparate impact attacks}
As disparate impact attacks, the final objective of the attacker is to increase the error for the privileged unfavorable and unprivileged favorable samples causing a bigger proportion of privileged samples to be assigned the positive outcome and having a bigger proportion of unprivileged samples being classified in the negative class.

\subsubsection{Perfect-Knowledge (PK) White-Box Attack setting}
In this first experiment, we studied the case where the attacker has perfect knowledge of the learned function and also about the input data.

The following experiments were executed by using the Eqs. \ref{eq:obj-pois}, \ref{eq:poisoning_problem}. In this set up, the inner problem is minimized for the set of privileged and favored samples, whereas the outer problem is maximized for both the privileged unfavorable and the unprivileged favorable groups. Also, this function gets minimized for the unprivileged favorable samples. We use a balancing factor $\lambda = 1$ to set the same relative weight of both parts in the outer function.


A synthetic data set is used to empirically test the capabilities of the stated technique depending of level of original disparate found in training data.

Data is generated using the same approach used by \cite{zafar2015fairness}. Specifically, we generated 4,000 binary class labels uniformly at random. For each label, a 2-dimensional user feature vector is assigned by drawing samples from two different Gaussian distributions:
$p(x|y=1) = N([2;2], [5, 1; 1, 5]$ and $p(x|y=-1) = N([\mu_1;\mu_2], [10, 1; 1,3])$ where $\mu_1, \mu_2$ are calculated from parametrized euclidean distance. A parameter $Euc_{distance}$ is used to parametrize the euclidean distance between the centroids of the distributions for the privileged and unprivileged groups so different degrees of difference are tested in the experiments executed afterwards.

Then, a sample's sensitive attribute is calculated from a Bernoulli distribution where $p(z=1) = p(x'| y=1) /(p(x'| y=1) + p(x'| y=0))$ where $x' = [cos(\phi) - sin(\phi); sin(\phi), cos(\phi)]x $ corresponds to a rotated version of the feature vector,$x$.

\begin{figure}[H]
  \centering
      \includegraphics[width=0.95\textwidth]{syntetic_data.png}
  \caption{Examples of generated synthetic data sets for different values of $Euc_{distance}$ between groups}.
  \label{fig:Synthetic_dataset}
\end{figure}

Generating data using the mentioned formula, the data set depicted in Figure \ref{fig:Synthetic_dataset} was obtained. Where the feature vector $x$ is represented in the horizontal and vertical axes, color represents the assigned label and symbol the sensitive attribute $z$.

To implement the attack, the following algorithm was followed:
\begin{algorithm}[H]
\caption{White-Box disparate impact attack algorithm}\label{dimp_attack}
\begin{algorithmic}[1]
\Procedure{White Box Disparate impact attack}{data, $M_{original}$}\\
\State $D_{tr}, D_{val}, D_{test} \gets splitData(data)$\\

\State $M_{original} \gets trainNewModelLogReg(D_{tr})$\\

\State $u^- \gets getUnprivilegedDenied(D_{tr}, D_{val})$
\State $u^+ \gets getUnprivilegedGranted(D_{tr}, D_{val})$
\State $p^+ \gets getPrivilegedDenied(D_{tr}, D_{val})$
\State $p^- \gets getPrivilagedGranted(D_{tr}, D_{val})$\\

\State $D_{tr}: \gets u^- \cup p^+$
\State $D_{val} \gets u^+ \cup p^-$\\

\State $samples_{poisoned} \gets generateSamples(M_{original}, D_{tr}, D_{val})$\\

\State $M_{poisoned} \gets retrainModel(M_{original}, D_{tr} + samples_{poisoned})$
\EndProcedure
\end{algorithmic}
\end{algorithm}

In this example, the poisoned model is the result of training the original model with the tranining dataset extended by the poisoned samples. $M_{original}$ corresponds to a Logistic Regression classifier.

In the algorithm, the poisoned examples $poisoned_{samples}$ are generated by optimizing Eq. \ref{eq:obj-pois} and Eq. \ref{eq:poisoning_problem} such that the loss $\set L$ gets minimized for the training data and maximized for the validation set.

Results shown in Figure \ref{fig:dimp_attack_white} were obtained by comparing the performance obtained by a model trained in the original data with the performance of the model trained on the poisoned data. The obtained performance is evaluated in the function \texttt{evaluate()} according to the following metrics:


\begin{itemize}
\item{ \textbf{a)Accuracy} The accuracy on test obtained by the poisoned model is similar and correlated to the accuracy obtained by a model trained in the original data. It's important to denote that the separability of the generated data is also highly correlated with the euclidean distance between the groups, creating this effect.}

\item {\textbf{b) Disparate impact} Maximum disparate introduced on the model's predictions highly correlates with initial disparate impact observed in the training data.}

\item {\textbf{c) FNR privileged} False Negative Rate for the privileged group of samples.}

\item {\textbf{d) FNR unprivileged} False Negative Rate for the unprivileged group of samples.}

\item {\textbf{e) FPR privileged} False Positive Rate for the unprivileged group of samples.}

\item {\textbf{f) FPR unprivileged} False Positive Rate for the unprivileged group of samples.}
\end{itemize}


\begin{figure}[H]
        \centering
        \includegraphics[width=0.8
        \textwidth]{dimp_attack.png}
    \caption{Performance comparison of original classifier and poisoned classifier for the disparate impact adversarial attack.}
    \label{fig:dimp_attack_white}
\end{figure}

Figure \ref{fig:dimp_attack_white} shows the average of the obtained results in 10 runs of the adversarial disparate impact attack for different values of distance between the groups on the synthetic data. $X$ axis shows the initial distance between the data groups where $Y$ axis shows the obtained value for each metric.\\

As can be seen, the poisoned model increases the initial disparate impact observed in the input data for all the settings as an effect of increased FNR for the unprivileged group and an increased FPR for the privileged group.

\subsubsection{Limited-Knowledge (LK) Gray-Box Attack setting}
This experiment corresponds to the setting where the attacker has partial knowledge of the scenario: has access to the original data, knows the task the system is designed to solve an the sensitive attributes of the samples but doesn't have access to the concrete model and its learned function. Therefore, the attacker will optimize the samples for a surrogate model, trained with the same data, that will approximate the real one. After, we train the original model with the new poisoned samples to perform the attack. This approach can be used due to the transferability of adversarial attacks, as was initially explained in \cite{demontis2018adversarial}.

To execute this experiment, we first trained $M_{original}$, a linear Support Vector Machines classifier. After, we train a surrogate classifier $M_{surrogate}$, a Logistic Regression classifier, with the same data and the attack is optimized for $M_{surrogate}$. The performance of the attack is measured by retraining the original model with the data optimized on the surrogate model. The experiments prove that even in this set up, the attack could cause drastic change of performance for the population groups:

\begin{algorithm}[H]
\caption{Gray-Box disparate impact attack algorithm}\label{euclid}
\begin{algorithmic}[1]
\Procedure{Gray-Box Disparate Impact attack}{data, $M_{original}$}\\
\State $D_{tr}, D_{val}, D_{test} \gets splitData(data)$\\

\State $M_{original} \gets trainNewModelSVM(training)$\\
\State $M_{surrogate} \gets trainNewModelLogReg(training)$\\

\State $u^- \gets getUnprivilegedDenied(D_{tr}, D_{val})$
\State $u^+ \gets getUnprivilegedGranted(D_{tr}, D_{val})$
\State $p^+ \gets getPrivilegedDenied(D_{tr}, D_{val})$
\State $p^- \gets getPrivilagedGranted(D_{tr}, D_{val})$\\

\State $D_{tr}: \gets u^- \cup p^+$
\State $D_{val} \gets u^+ \cup p^-$\\

\State $samples_{poisoned} \gets generateSamples(M_{surrogate}, D_{tr}, D_{val})$\\

\State $M_{poisoned} \gets retrainModel(M_{original}, D_{tr} + samples_{poisoned})$
\EndProcedure
\end{algorithmic}
\end{algorithm}


\begin{figure}[H]
        \centering
        \includegraphics[width=0.6
        \textwidth]{dimp_attack_gray.png}
    \caption{Performance comparison of original classifier and poisoned classifier for the disparate impact adversarial attack with Limited Knowledge (LK) setting.}
    \label{fig:dimp_attack_gray}
\end{figure}


%%DISPARATE MISTREATMENT ATTACK
\subsection{Disparate mistreatment attacks}
As disparate mistreatment attack, the final objective of the attacker is to increase the error for the unprivileged and decrease it for the privileged samples causing a bigger bigger disparate between both groups. To maximize the disparate mistreatment introduced by the trained models, the inner problem is minimized for the set of all the privileged samples, whereas the outer problem is minimized for all the privileged ones, for that, we don't use any data in the second term of the outer problem ($\lambda = 0$).

For this experiment, we used a real world dataset, commonly used in the field of Algorithmic Fairness: The ProPublica data includes data collected about the use of the COMPAS risk assessment tool in Broward County, Florida Angwin et al. (2016). It includes information such as the number of juvenile felonies and the charge degree of the current arrest for 6,167 individuals, along with sensitive attributes race and sex. Data is pre-processed according to the filters given in the original analysis \cite{ProPublica_article}. Each individual has a binary “recidivism” outcome, that is the prediction task, indicating whether they were rearrested within two years after the first arrest (the charge described in the data).

In this data set, \textit{sex} and \textit{race} are the protected attributes, both of them having value $1$ for the privileged groups. Favorable outcome corresponds to the label with value $1$, corresponding to \textit{low risk} assignations.

Using this data, we tested the \textit{Perfect-Knowledge (PK)} and \textit{Limited-Knowledge (LK)} settings as was done in the experiments above.

\subsubsection{Perfect-Knowledge (PK) White-Box Attack setting}
To be done

\begin{table}[H]
\centering
\begin{tabular}{l|l|l|l|l|l|}
\cline{2-6}
                                          & Accuracy & \begin{tabular}[c]{@{}l@{}}FNR\\ privileged\end{tabular} & \begin{tabular}[c]{@{}l@{}}FNR\\ unprivileged\end{tabular} & \begin{tabular}[c]{@{}l@{}}FPR\\ privileged\end{tabular} & \begin{tabular}[c]{@{}l@{}}FPR\\ unprivileged\end{tabular} \\ \hline
\multicolumn{1}{|l|}{Original classifier} & 65.65\%  & 20.93\%                                                  & 31.33\%                                                       & 71.43\%                                                  & 32.09\%                                                    \\ \hline
\multicolumn{1}{|l|}{Poisoned classifier} & 54.08\%  & 0.0\%                                                    & 100\%                                                      & 0.0\%                                                    & 100\%                                                      \\ \hline
\end{tabular}
\caption{Obtained results on the disparate mistreatment attack on the Perfect-Knowledge setting.}
\label{tab:compas_results_white}
\end{table}

\subsubsection{Limited-Knowledge (LK) Gray-Box Attack setting}
To be done
\begin{table}[H]
\centering
\begin{tabular}{l|l|l|l|l|l|}
\cline{2-6}
                                          & Accuracy & \begin{tabular}[c]{@{}l@{}}FNR\\ privileged\end{tabular} & \begin{tabular}[c]{@{}l@{}}FNR\\ unprivileged\end{tabular} & \begin{tabular}[c]{@{}l@{}}FPR\\ privileged\end{tabular} & \begin{tabular}[c]{@{}l@{}}FPR\\ unprivileged\end{tabular} \\ \hline
\multicolumn{1}{|l|}{Original classifier} & 62.81\%  & 29.46\%                                                  & 50\%                                                       & 54.29\%                                                  & 22.84\%                                                    \\ \hline
\multicolumn{1}{|l|}{Poisoned classifier} & 54.08\%  & 0.0\%                                                    & 100\%                                                      & 0.0\%                                                    & 100\%                                                      \\ \hline
\end{tabular}
\caption{Obtained results on the disparate mistreatment attack on the Limited-Knowledge (LK) setting.}
\label{tab:compas_results_gray}
\end{table}

The results obtained in Table \ref{tab:compas_results_gray} show how the optimized attack maximizes the differences of errors. This effect is caused because of the high dimentionality of the data which facilitates the obtention of adversarial samples that maximize the impact.


==> old_sections/05-related-work.tex <==
%!TEX root = paper.tex

\section{Related work}\label{sec:related-work}

\subsection{Gradient-based attacks}

This work is based in an optimization framework widely used in the literature of Adversarial Machine Learning for crafting poisoning attacks. This framework is known as Gradient-based Optimization Algorithm and has been referenced by different research articles exploring poisoning attacks \cite{biggio2012poisoning,Mei2015UsingML,muozgonzlez2017poisoning,jagielski2018manipulating,demontis2018adversarial}.

Such framework is used to solve the bilevel optimization problem given by Eqs. \ref{eqObjective1}\ref{eqObjective2} and requires to compute the gradient of the classification function learned by the classifier. As result of solving the optimization problem, optimal attack samples can be obtained by iteratively optimizing one attack point at a time \cite{Xiao_2015_feature_selection}.


\subsection{Adversarial attacks in Algorithmic Fairness}
Adversarial attacks have been considered in recent articles within the domain of Algorithmic Fairness. In that regard, authors from \cite{Rastegarpanah_2019,Kulynych_2020} explored the usage of poisoning attacks for crafting antidote samples that can are incorporated in the training set to reduce the unfairness of the system. When the first approach proposes a method to be applied on recommender systems based on matrix factorization, the later is also based in the Gradinet-based Optimization framework used in this work. More recently, authors of \cite{delobelle2020ethical} proposed a framework leveraging evasion attacks from adversarial machine learning to perform adversarial retraining with new examples unseen by the model, proving that it helped into mitigating unfairness with respect the protected attributes.

\subsection{Optimization-based approaches to remove algorithmic unfairness}
In addition to this, authors of \cite{zafar2015fairness,Zafar_2017} propose an optimization problem so solve the inherent trade-off between accuracy and fairness. In their work, they approached the problem through an alternative definition of fairness based in covariance between the users’
sensitive attributes and the signed distance between the feature vectors of misclassified users and the classifier decision
boundary.


==> old_sections/06-conclusions.tex <==
%!TEX root = paper.tex

\section{Conclusions}\label{sec:conclusions}

The obtained results show the feasibility of a new kind of adversarial attacks crafted with the objective of increasing the disparate impact at the level of the system predictions, regardless of the initial disparate impact reflected in the data for certain groups.
%
With the only additional requirement for the attacker to know the privileged and unprivileged conditions of the existing samples, this knowledge can be used together with state of the art techniques in adversarial machine learning to cause or increase the inequities in the system.

% Future work:
Although experiments are done using a specific technique based on a poisoning attack, other techniques can be certainly considered. More advanced approaches such as causality-based techniques could be explored, although this exceeds the demonstration purpose of this work.


==> removed.tex <==

% Removed material

\section{Algorithmic Fairness}

During the past few years, the intersection between data mining, machine learning and fairness domains has received an increasing attention by the research community. In this context, the work done for task of quantifying inequities, named algorithmic fairness, resulted in a multitude of metrics to quantify fairness.\\

The existing metrics of fairness for classification fall in two categories:  \textit{Individual metrics} and \textit{Group metrics} depending if the goal is to require the system to give similar predictions to individuals that are considered similar or the objective is that the system treats groups equally. The groups are often calculated in the bases of sensible attributes that are legally recognized as protected classes.\\

In general, approaches to algorithmic fairness are based on a specific distribution of the feature space. As indicated by \cite{Pedreschi_2012}, this distribution can be expressed in the form of a contingency table that divides the features space in terms of the groups found in the data. Groups are calculated with respect to a protected attribute $A$ and a target variable $Y$, for which some of the possible values are considered more beneficial than others. Following this ideas, for the simple case of binary classification and two groups, the feature space is divided as depicted in Table \ref{tab:fairness_feature_space}.


\begin{table}[ht!]
\centering
\begin{tabular}{llllll}
                                                           &                                  & \multicolumn{2}{c}{{\ul \textbf{benefit}}}                 &    &  \\ \cline{3-4}
                                                           & \multicolumn{1}{l|}{}            & \multicolumn{1}{l|}{denied} & \multicolumn{1}{l|}{granted} &    &  \\ \cline{2-5}
\multicolumn{1}{c|}{\multirow{2}{*}{{\ul \textbf{group}}}} & \multicolumn{1}{l|}{unprivileged}   & \multicolumn{1}{l|}{$u^-$}      & \multicolumn{1}{l|}{$u^+$}       & $n_1$ &  \\ \cline{2-5}
\multicolumn{1}{c|}{}                                      & \multicolumn{1}{l|}{privileged} & \multicolumn{1}{l|}{$p^-$}      & \multicolumn{1}{l|}{$p^+$}       & $n_2$ &  \\ \cline{2-5}
                                                           & \multicolumn{1}{l|}{}            & \multicolumn{1}{l|}{$m_1$}     & \multicolumn{1}{l|}{$m_2$}      & $n$  &
\end{tabular}
\medskip
\caption{Contingency table. Distribution of feature space in algorithmic fairness literature}
\label{tab:fairness_feature_space}
\end{table}


As proposed in the literature \cite{alex2016fair,Zafar_2017,feldman2015}, fairness functions are defined by using the criteria of \textit{disparate impact} and \textit{disparate mistreatment} depending on the final goal of the metric.

Given $X$, a feature vector representing individuals; $A$, a sensitive attribute; $C$, a predictor and $Y$ a target variable, the stated criteria are defined as follows:
\begin{itemize}
    \item {\textbf{Disparate impact:} Requires $C$ independent of $A$ ($C\perp A$).\\ Implies that for all groups $a$, $b$ and all values $y$, $P_a (C=y) = P_b(C=y) $.\\
    This criterion ignores possible correlations between $Y$ and $A$.\\ The case of the perfect predictor ($C = Y$) is in general not accepted in most cases, where initial rates for $Y$ values across groups are not equalized. \\
    Examples of metrics based in this criteria are: \textit{demographic parity} and \textit{statistical parity}.}\\

    \item {\textbf{Disparate mistreatment:} Requires $C$ independent of $A$ conditional on $Y$ ($C\perp A | Y$)}.\\
    This criteria incentives to reduce errors uniformly in all groups. The case of the perfect predictor $C = Y$ is allowed and corresponds to the ideal scenario. Introduced first in \cite{Zafar_2017}, examples of metrics based on it are: \textit{true positive ratio}, \textit{false positive ratio}, \textit{true positive ratio} and \textit{average odds difference} \cite{Zafar_2017} that accounts for differences in both metrics within the groups at the same time.\\
\end{itemize}

The impossibility theorem of satisfying any both criteria at the same time is already known. In  \cite{alex2016fair,kleinberg2016}, authors demonstrated the unfeasibility of achieving fairness according both definitions at the same time, when the base rates for the different groups is different.
